Lattice Dynamics Calculations based on Density-functional Perturbation Theory in Real Space

A real-space formalism for density-functional perturbation theory (DFPT) is derived and applied for the computation of harmonic vibrational properties in molecules and solids. The practical implementation using numeric atom-centered orbitals as basis functions is demonstrated exemplarily for the all-electron Fritz Haber Institute ab initio molecular simulations (FHI-aims) package. The convergence of the calculations with respect to numerical parameters is carefully investigated and a systematic comparison with finite-difference approaches is performed both for finite (molecules) and extended (periodic) systems. Finally, the scaling tests and scalability tests on massively parallel computer systems demonstrate the computational efficiency.

==> Makefile <==
base_name := CPC
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))

%.dvi: %.tex
	$(MAKE) -C figures
	latex --interaction=nonstopmode $<
	latex --interaction=nonstopmode $<
#	makeindex -s index-style.ist $*.idx
	bibtex $*.aux
	latex --interaction=nonstopmode $<
	latex --interaction=nonstopmode $<

%.pdf: %.tex
	$(MAKE) -C figures
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<
#	makeindex -s index-style.ist $*.idx
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<

%.ps: %.dvi
	dvips $<

all: $(base_name).pdf  
	(evince $(base_name).pdf  &)
pdf: $(base_name).pdf
ps:  $(base_name).ps
display: 
	evince $(base_name).pdf 


$(base_name).pdf: $(base_name).tex $(base_name).bib 

figures:
	$(MAKE) -C figures

dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

semiclean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib

figuresclean:
	$(MAKE) -C figures clean

clean:
	$(MAKE) semiclean
	$(MAKE) figuresclean	

.PHONY: clean figuresclean semiclean backup


==> figures/Makefile <==
source_asy := $(wildcard src/*.asy)
cube_data  := $(wildcard data/*.cube)
pdf_images := $(patsubst src/%.asy,pdf/%.pdf,$(source_asy))  \
							$(patsubst data/%.cube,pdf/%.pdf,$(cube_data))
eps_images := $(patsubst src/%.asy,eps/%.eps,$(source_asy))
png_images := $(patsubst src/%.asy,png/%.png,$(source_asy))

eps/%.eps: src/%.asy
	asy -render=0 $< -o $@

eps/%.eps: tga/%.tga
	convert tga/plot.tga $@

png/%.png: src/%.asy
	asy -render=0 -f png $< -o $@

png/%.png: tga/%.tga
	convert tga/plot.tga $@

pdf/%.pdf: eps/%.eps
	epstopdf --outfile=$@ $<

pdf/%.pdf: tga/%.tga
	convert tga/plot.tga $@

tga/wp-%.tga: data/wp-%.cube
	vmd -f $< -e src/dftb-orbitals.vmd -dispdev text -eofexit

tga/eigenstate_%.tga: data/eigenstate_%.cube
	vmd -f $< -e src/aims-orbitals.vmd -dispdev text -eofexit

all: $(pdf_images) $(eps_images) #$(png_images) 

clean:
	#rm -f *~ src/*~ eps/*.eps png/*.png pdf/*.pdf tga/*.tga

.PHONY: clean


==> macros.tex <==
\renewcommand{\vec}[1]{{\bf #1}}
\renewcommand{\v}[1]{{\bf #1}}
\newcommand{\intint}{\int\!\!\!\int}
\newcommand{\eref}[1]{(\ref{#1})}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\def\hOa{\overline{{\hat O}}}
\def\hS{{\hat S}}
\def\hO{{\hat O}}
\def\hH{{\hat H}}
\def\half{\frac{1}{2}}
\def\la{{\langle\, }}
\def\ra{{\,\rangle }}
\def\p{\,|\,}
\def\KS{_{\rm KS}}
\def\EET{_{\rm EET}}
